typedKanren: Statically Typed Relational Programming with Exhaustive Matching in Haskell

We present a statically typed embedding of relational programming (specifically a dialect of miniKanren with disequality constraints) in Haskell. Apart from handling types, our dialect extends standard relational combinator repertoire with a variation of relational matching that supports static exhaustiveness checks. To hide the boilerplate definitions and support comfortable logic programming with user-defined data types we use generic programming via GHC.Generics as well as metaprogramming via Template Haskell. We demonstrate our dialect on several examples and compare its performance against some other known implementations of miniKanren.

==> sections/5-examples.tex <==
\section{Examples}
\label{sec:examples}

Here we can present some examples and, perhaps, benchmarks,
showing how our implementation is on par or better than some others.

